When is the set of embeddings finite up to isotopy?

Given a manifold N and a number m, we study the following question: is the set of isotopy classes of embeddings N->S^m finite? In case when the manifold N is a sphere the answer was given by A. Haefliger in 1966. In case when the manifold N is a disjoint union of spheres the answer was given by D. Crowley, S. Ferry and the author in 2011. We consider the next natural case when N is a product of two spheres. In the following theorem, FCS(i,j) is a concrete subset of the integer lattice depending only on the parity of i and j which is defined in the paper. Theorem. Assume that m>2p+q+2 and m<p+3q/2+2. Then the set of isotopy classes of smooth embeddings S^p x S^q -> S^m is infinite if and only if either q+1 or p+q+1 is divisible by 4, or there exists a point (x,y) in the set FCS(m-p-q,m-q) such that (m-p-q-2)x+(m-q-2)y=m-3. Our approach is based on a group structure on the set of embeddings and a new exact sequence, which in some sense reduces the classification of embeddings S^p x S^q -> S^m to the classification of embeddings S^{p+q} |_| S^q -> S^m and D^p x S^q -> S^m. The latter classification problems are reduced to homotopy ones, which are solved rationally.

==> Fig01.tex <==

%\input pictex
\beginpicture % by PiCTeX CAD
\setcoordinatesystem units <0.600mm,0.600mm>
\setplotarea x from -60 to 60, y from -40 to 20
\put {Figure 1} at 0 -40.000

%\grid 1 1

\setcoordinatesystem units <0.600mm,0.600mm> point at 30 0
\setplotarea x from -30 to 30, y from -35 to 20

%\grid 1 1

\setsolid \setplotsymbol ({\fiverm.}) \circulararc 336.650 degrees
from -7.975 -3.967 center at -0.000 -10.000 \circulararc 336.650
degrees from 7.975 -1.033 center at -0.000 5.000 \put {$S^0 \times
S^1 \to S^3$} at 0 -26.000 \put {a} at 0 -34.000

\setcoordinatesystem units <0.600mm,0.600mm> point at -30 0
\setplotarea x from -30 to 30, y from -35 to 20

%\grid 1 1

\setsolid
\setplotsymbol ({\fiverm.})
\circulararc 3.423 degrees from -8.354 5.471 center at -11.020 -16.690
\circulararc 34.433 degrees from 8.944 -6.708 center at -11.020 -16.690
\circulararc 6.253 degrees from -6.422 10.241 center at -11.020 -16.690
\circulararc 36.084 degrees from 13.416 -4.472 center at -11.020 -16.690
\circulararc 36.084 degrees from -10.581 -9.383 center at -8.944 17.889
\circulararc 6.253 degrees from 12.080 0.441 center at -8.944 17.889
\circulararc 34.433 degrees from -10.282 -4.392 center at -8.944 17.889
\circulararc 3.423 degrees from 8.915 4.500 center at -8.944 17.889
\circulararc 3.423 degrees from -0.560 -9.970 center at 19.964 -1.198
\circulararc 34.433 degrees from 1.337 11.100 center at 19.964 -1.198
\circulararc 6.253 degrees from -5.658 -10.682 center at 19.964 -1.198
\circulararc 36.084 degrees from -2.835 13.855 center at 19.964 -1.198
\circulararc 33.373 degrees from 12.083 -13.748 center at 4.472 -8.944
\circulararc 77.104 degrees from 13.470 -8.770 center at 11.801 -10.531
\circulararc 39.888 degrees from 9.342 -12.449 center at 4.472 -8.944
\circulararc 42.759 degrees from 12.083 -13.748 center at 9.053 -16.600
\circulararc 180.000 degrees from -4.472 -13.416 center at 4.472 -8.944
\circulararc 180.000 degrees from -9.383 10.581 center at -9.982 0.599
\circulararc 180.000 degrees from 13.855 2.835 center at 5.510 8.345
\circulararc 180.000 degrees from 0.000 -11.180 center at 4.472 -8.944
\circulararc 180.000 degrees from -9.682 5.590 center at -9.982 0.599
\circulararc 180.000 degrees from 9.682 5.590 center at 5.510 8.345
\put {$B^2$} at 18.566 -10.728
\put {$S^1 \times S^1 \to S^3$} at 0 -26.000
\put {b} at 0 -34.000
\endpicture
%\bye

